Enabling Quartile-based Estimated-Mean Gradient Aggregation As Baseline for Federated Image Classifications

Federated Learning (FL) has revolutionized how we train deep neural networks by enabling decentralized collaboration while safeguarding sensitive data and improving model performance. However, FL faces two crucial challenges: the diverse nature of data held by individual clients and the vulnerability of the FL system to security breaches. This paper introduces an innovative solution named Estimated Mean Aggregation (EMA) that not only addresses these challenges but also provides a fundamental reference point as a $\mathsf{baseline}$ for advanced aggregation techniques in FL systems. EMA's significance lies in its dual role: enhancing model security by effectively handling malicious outliers through trimmed means and uncovering data heterogeneity to ensure that trained models are adaptable across various client datasets. Through a wealth of experiments, EMA consistently demonstrates high accuracy and area under the curve (AUC) compared to alternative methods, establishing itself as a robust baseline for evaluating the effectiveness and security of FL aggregation methods. EMA's contributions thus offer a crucial step forward in advancing the efficiency, security, and versatility of decentralized deep learning in the context of FL.

==> ICASSP2024_Paper_Templates/sections/alg2.tex <==

\begin{tikzpicture}[scale=0.6]
\begin{axis}[
	every axis plot post/.style={/pgf/number format/fixed},
	ybar,
	bar width=15pt,
	x=3cm,
	ymin=0,
	axis on top,
	ylabel={Gradients within normal distribution (\%)},
	ymax=90,
	xtick=data,
	enlarge x limits=0.7,
	symbolic x coords={CIFAR10, MINST},
	visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.0) -- (rel axis cs:1,1.0);
        },
    nodes near coords={%
            \pgfmathprintnumber{\rawy}% Print unclipped values
        },
        every node near coord/.append style={font=\scriptsize},
    axis lines*=left,
    clip=false,
    legend columns=1,
    legend image code/.code={%
      \draw[#1] (0cm,-0.1cm) rectangle (0.5cm,0.1cm);
    },
    legend style={at={(0.05,1)},anchor=north west}
    ]

\addplot [pattern = north east lines, pattern color=red] coordinates {(MINST,78.36) (CIFAR10, 78.3)};
 
\addplot [pattern = north west lines, pattern color=black] coordinates {(MINST,80.25) (CIFAR10,80.26)};
%\addplot [pattern = north west lines, pattern color=blue] coordinates {(unreplicated,13.39136) (replicated,11.10803)};




%\legend{Chios,Kafka-SingleProducer,Kafka-MultiProducer,Fabric}
%\legend{Chios,Kafka,Fabric}
\end{axis}
\node at (4.8,6.9) {{\tiny SW}};
\node at (5.4,7.0) {{\tiny AD}};

\node at (1.8,6.9) {{\tiny SW}};
\node at (2.4,7.0) {{\tiny AD}};
\end{tikzpicture}



==> ICASSP2024_Paper_Templates/sections/intr.tex <==
\section{Introduction} \label{introduction} 

Federated Learning (FL) is a pioneering approach that enables the training of models across multiple devices or clients while keeping their data localized. In traditional machine learning, data is typically collected from various sources and centralized for model training. FL, however, allows training models directly on the clients without the need to transfer raw data to a central server. Then gradient aggregation is used to combine the gradients computed by individual clients to update the global model. This method ensures the confidentiality of sensitive data held by each client while collectively improving model performance. Despite its advancements, the effectiveness of FL can be hindered by certain challenges and considerations. One notable challenge is the presence of data heterogeneity, which refers to whether the data distribution is independent and identically distributed (IID) or non-IID in nature. The intricacy of the situation may complicate the process of gradient aggregation from different clients. Another significant challenge pertains to model security. Federated learning systems encounter the risk that clients could be prone to different types of security breaches, including susceptibility to various forms of poisoning attacks. These possible security weaknesses require careful monitoring and strong protective measures. For instance, an emerging threat involves the possibility of a gradient inversion attack, which can lead to the convergence of a trained model from manipulated gradients. This type of threat emphasizes the significance of strengthening FL systems to guard against potential privacy breaches, highlighting the necessity for strong defense mechanisms.

Numerous robust strategies have been put forth to withstand diverse attacks or Byzantine failures, including techniques like median \cite{yin2018byzantine}, trimmed mean \cite{yin2018byzantine}, and krum \cite{blanchard2017machine}. However, almost all the aggregation solutions have difficulties addressing the first challenge because aggregation takes place on the server side, while data heterogeneity occurs on the client side. Furthermore, the absence of standardized benchmarks compounds the challenge of assessing the efficacy of an aggregation method. Our present requirements encompass the deployment of an integrated approach capable of concurrently fulfilling the ensuing objectives: 1), establishing a baseline for assessing the existing aggregation solutions. 2), upholding the inviolability of model security, 3), identifying instances of data heterogeneity, 4), augmenting the overall efficiency of aggregation, and importantly.


Inspired by Luo et al. \cite{luo2018optimally}, wherein they propounded a theoretical algorithm for inferring the mean of a dataset by leveraging statistical measures such as the first quartile, third quartile, and median of the sample data, we offer an innovative estimated mean aggregation (EMA) methodology. This methodology serves as a discerning instrument (e.g., baseline) for the comprehensive evaluation of diverse advanced aggregation protocols. In select scenarios, the employment of the EMA assumes the role of a foundational aggregation technique. Its role as a baseline opens the door to thorough examination and comparative analysis of more complex aggregation techniques in comparison to this foundational baseline, enabling an assessment of their effectiveness in enhancing the performance metrics of FL.

One of the key advantages of EMA is its ability to mitigate the adverse effects of malicious outliers in gradient aggregation through the trimmed means to guarantee \textit{model security}. By computing the Interquartile Range (IQR) as the difference between the third quartile ($q3$) and the first quartile ($q1$), denoted as $IQR = q3 - q1$, and subsequently selecting a trimming percentage $t$ to determine the proportion of data points to be trimmed, the method offers a systematic means to control the influence of malicious outliers. The permissible range of outlier values to be trimmed, $Trim\ Range = IQR \times \frac{t}{100}$, serves as a parameter to identify the extent of outlier removal. This leads to the formulation of the percentage of malicious outliers,
% which is formulated as the percentage of outliers 
$p = \frac{Trim\ Range}{Max(X) - Min(X)} \times 100$. 
After removing the outliers, the remaining gradients are then employed to compute an estimated mean. By addressing malicious outliers in this systematic manner, the method enhances the resilience of data analysis and contributes to the development of more robust statistical techniques against intentional gradient manipulation.

In addition to addressing the challenge of evaluating a federated model across non-IID or IID datasets (identifying data heterogeneity), we present a comprehensive solution that leverages the unique characteristics of each client's data distribution. This solution involves assessing the performance of the trained model on each individual client, thereby enabling an insightful analysis of the model's adaptability to diverse data scenarios. To achieve this, we introduce the method as a cornerstone \textcolor{red}{(comprehensive, insightful, and cornerstone. They are all strong words, but with limited description of the method)} of our approach. This method allows us to evaluate the model's performance within the context of each client's dataset. By retrieving the model specific to each client and utilizing the Mean Squared Error (MSE) loss criterion, we accurately measure the model's predictive capability and its fit to the respective data. 


The key contributions of this work include:
\begin{itemize}[itemsep=-1pt] % Adjust the value as needed
\item We have introduced a novel and efficient method for estimated mean aggregation, termed EMA, which streamlines gradient aggregation while concurrently minimizing communication overhead. Our EMA aggregation approach also ensures the preservation of model security.
\item We devised and executed a comprehensive model evaluation algorithm tailored for the assessment of trained models across datasets characterized by diverse attributes. This algorithm facilitates a meticulous examination of model adaptability in varying data scenarios, enabling the identification of heterogeneous datasets.
\item We evaluated EMA in comparison to other advanced aggregation rules across varying biomedical datasets. The results show that EMA consistently outperforms its counterparts in terms of convergence speed and model accuracy. This finding underscores the robustness and effectiveness of EMA as a baseline aggregation technique.


\end{itemize}

==> sections/alg2.tex <==

\begin{tikzpicture}[scale=0.6]
\begin{axis}[
	every axis plot post/.style={/pgf/number format/fixed},
	ybar,
	bar width=15pt,
	x=3cm,
	ymin=0,
	axis on top,
	ylabel={Gradients within normal distribution (\%)},
	ymax=90,
	xtick=data,
	enlarge x limits=0.7,
	symbolic x coords={CIFAR10, MINST},
	visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.0) -- (rel axis cs:1,1.0);
        },
    nodes near coords={%
            \pgfmathprintnumber{\rawy}% Print unclipped values
        },
        every node near coord/.append style={font=\scriptsize},
    axis lines*=left,
    clip=false,
    legend columns=1,
    legend image code/.code={%
      \draw[#1] (0cm,-0.1cm) rectangle (0.5cm,0.1cm);
    },
    legend style={at={(0.05,1)},anchor=north west}
    ]

\addplot [pattern = north east lines, pattern color=red] coordinates {(MINST,78.36) (CIFAR10, 78.3)};
 
\addplot [pattern = north west lines, pattern color=black] coordinates {(MINST,80.25) (CIFAR10,80.26)};
%\addplot [pattern = north west lines, pattern color=blue] coordinates {(unreplicated,13.39136) (replicated,11.10803)};




%\legend{Chios,Kafka-SingleProducer,Kafka-MultiProducer,Fabric}
%\legend{Chios,Kafka,Fabric}
\end{axis}
\node at (4.8,6.9) {{\tiny SW}};
\node at (5.4,7.0) {{\tiny AD}};

\node at (1.8,6.9) {{\tiny SW}};
\node at (2.4,7.0) {{\tiny AD}};
\end{tikzpicture}



==> sections/intr.tex <==
\section{Introduction} \label{introduction} 

Federated Learning (FL) is a pioneering approach that enables the training of models across multiple devices or clients while keeping their data localized. In traditional machine learning, data is typically collected from various sources and centralized for model training. FL, however, allows training models directly on the clients without the need to transfer raw data to a central server. Then gradient aggregation is used to combine the gradients computed by individual clients to update the global model. This method ensures the confidentiality of sensitive data held by each client while collectively improving model performance. Despite its advancements, the effectiveness of FL can be hindered by certain challenges and considerations. One notable challenge is the presence of data heterogeneity, which refers to whether the data distribution is independent and identically distributed (IID) or non-IID in nature. The intricacy of the situation may complicate the process of gradient aggregation from different clients. Another significant challenge pertains to model security. Federated learning systems encounter the risk that clients could be prone to different types of security breaches, including susceptibility to various forms of poisoning attacks. These possible security weaknesses require careful monitoring and strong protective measures. For instance, an emerging threat involves the possibility of a gradient inversion attack, which can lead to the convergence of a trained model from manipulated gradients. This type of threat emphasizes the significance of strengthening FL systems to guard against potential privacy breaches, highlighting the necessity for strong defense mechanisms.

Numerous robust strategies have been put forth to withstand diverse attacks or Byzantine failures, including techniques like median \cite{yin2018byzantine}, trimmed mean \cite{yin2018byzantine}, and krum \cite{blanchard2017machine}. However, almost all the aggregation solutions have difficulties addressing the first challenge because aggregation takes place on the server side, while data heterogeneity occurs on the client side. Furthermore, the absence of standardized benchmarks compounds the challenge of assessing the efficacy of an aggregation method. Our present requirements encompass the deployment of an integrated approach capable of concurrently fulfilling the ensuing objectives: 1), establishing a baseline for assessing the existing aggregation solutions. 2), upholding the inviolability of model security, 3), identifying instances of data heterogeneity, 4), augmenting the overall efficiency of aggregation, and importantly.


Inspired by Luo et al. \cite{luo2018optimally}, wherein they propounded a theoretical algorithm for inferring the mean of a dataset by leveraging statistical measures such as the first quartile, third quartile, and median of the sample data, we offer an innovative estimated mean aggregation (EMA) methodology. This methodology serves as a discerning instrument (e.g., baseline) for the comprehensive evaluation of diverse advanced aggregation protocols. In select scenarios, the employment of the EMA assumes the role of a foundational aggregation technique. Its role as a baseline opens the door to thorough examination and comparative analysis of more complex aggregation techniques in comparison to this foundational baseline, enabling an assessment of their effectiveness in enhancing the performance metrics of FL.

One of the key advantages of EMA is its ability to mitigate the adverse effects of malicious outliers in gradient aggregation through the trimmed means to guarantee \textit{model security}. By computing the Interquartile Range (IQR) as the difference between the third quartile ($q3$) and the first quartile ($q1$), denoted as $IQR = q3 - q1$, and subsequently selecting a trimming percentage $t$ to determine the proportion of data points to be trimmed, the method offers a systematic means to control the influence of malicious outliers. The permissible range of outlier values to be trimmed, $Trim\ Range = IQR \times \frac{t}{100}$, serves as a parameter to identify the extent of outlier removal. This leads to the formulation of the percentage of malicious outliers,
% which is formulated as the percentage of outliers 
$p = \frac{Trim\ Range}{Max(X) - Min(X)} \times 100$. 
After removing the outliers, the remaining gradients are then employed to compute an estimated mean. By addressing malicious outliers in this systematic manner, the method enhances the resilience of data analysis and contributes to the development of more robust statistical techniques against intentional gradient manipulation.

In addition to addressing the challenge of evaluating a federated model across non-IID or IID datasets (identifying data heterogeneity), we present a comprehensive solution that leverages the unique characteristics of each client's data distribution. This solution involves assessing the performance of the trained model on each individual client, thereby enabling an insightful analysis of the model's adaptability to diverse data scenarios. To achieve this, we introduce the method as a cornerstone \textcolor{red}{(comprehensive, insightful, and cornerstone. They are all strong words, but with limited description of the method)} of our approach. This method allows us to evaluate the model's performance within the context of each client's dataset. By retrieving the model specific to each client and utilizing the Mean Squared Error (MSE) loss criterion, we accurately measure the model's predictive capability and its fit to the respective data. 


The key contributions of this work include:
\begin{itemize}[itemsep=-1pt] % Adjust the value as needed
\item We have introduced a novel and efficient method for estimated mean aggregation, termed EMA, which streamlines gradient aggregation while concurrently minimizing communication overhead. Our EMA aggregation approach also ensures the preservation of model security.
\item We devised and executed a comprehensive model evaluation algorithm tailored for the assessment of trained models across datasets characterized by diverse attributes. This algorithm facilitates a meticulous examination of model adaptability in varying data scenarios, enabling the identification of heterogeneous datasets.
\item We evaluated EMA in comparison to other advanced aggregation rules across varying biomedical datasets. The results show that EMA consistently outperforms its counterparts in terms of convergence speed and model accuracy. This finding underscores the robustness and effectiveness of EMA as a baseline aggregation technique.


\end{itemize}
